StateAct: Enhancing LLM Base Agents via Self-prompting and State-tracking

Large language models (LLMs) are increasingly used as autonomous agents, tackling tasks from robotics to web navigation. Their performance depends on the underlying base agent. Existing methods, however, struggle with long-context reasoning and goal adherence. We introduce StateAct, a novel and efficient base agent that enhances decision-making through (1) self-prompting, which reinforces task goals at every step, and (2) chain-of-states, an extension of chain-of-thought that tracks state information over time. StateAct outperforms ReAct, the previous best base agent, by over 10% on Alfworld, 30% on Textcraft, and 7% on Webshop across multiple frontier LLMs. We also demonstrate that StateAct can be used as a drop-in replacement for ReAct with advanced LLM agent methods such as test-time scaling, yielding an additional 12% gain on Textcraft. By improving efficiency and long-range reasoning without requiring additional training or retrieval, StateAct provides a scalable foundation for LLM agents. We open source our code to support further research at https://github.com/ai-nikolai/stateact .

==> sections/1_introduction_alternative.tex <==
\section{Introduction}

Leveraging the built-in world and commonsense knowledge\footnote{Commonsense and world knowledge as explored by \citet{lauscher-etal-2020-common}, for example.} of large language models (LLMs) such as GPT, Gemini, and Mixtral \cite{brown2020language, Anil2023GeminiAF, jiang2024mixtral} to perform interactive reasoning tasks has become a key frontier in AI research. These LLM-powered ``AI Agents'' can now tackle a diverse range of complex, multimodal tasks \cite{durante2024agent}, including simulated robotics \cite{puig2018virtualhome, shridhar2021alfworld}, digital environments such as online shopping \cite{yao2023webshop}, operating system navigation \cite{liu2023agentbench}, and game-playing \cite{côté2019textworld, liu2023agentbench, prasad2024adaptasneededdecompositionplanning}.  

At the core of an LLM agent is the \textit{base agent}, such as Act \citep{huang2022language}, ReAct \citep{yao2023react}, and AdaPlanner \citep{Sun2023AdaPlannerAP}. Efforts to improve LLM agents typically build on these base agents but often require significant computational or human resources. For example, \citet{Wu2024StateFlowEL} rely on human-annotated rule sets, \citet{Sun2023AdaPlannerAP} require a code execution environment with meticulously designed prompts, and \citet{Fu2024AutoGuideAG} incorporate additional training data and retrieval-augmented generation (RAG). Other approaches involve fine-tuning on additional training data \citep{yang2024react}, leveraging test-time computation \citep{prasad2024adaptasneededdecompositionplanning, schroeder2024threadthinkingdeeperrecursive}, or both. Notably, many of these state-of-the-art methods use ReAct as their base agent.  

In this work, we introduce \textbf{StateAct}, a new base agent designed to address two key challenges in LLM agents: (i) maintaining adherence to the original instruction and goal over long interactions, and (ii) effectively utilizing long-context capabilities of LLMs \citep{Li2023LooGLECL, coelho2024dwell}. To address (i), we introduce \textit{self-prompting}, a mechanism that ensures the agent continuously reorients itself toward the main goal at every interaction step. To address (ii), we propose \textit{chain-of-states}, an extension of chain-of-thought reasoning that incorporates explicit state-tracking, enabling the agent to maintain awareness of critical environmental information such as location, inventory, and task progression.  

Our experiments show that StateAct achieves near state-of-the-art performance without using additional training data or additional tools, and significantly outperforms ReAct across multiple tasks and eight frontier LLMs of varying sizes. Specifically, StateAct improves performance over ReAct by more than 10\% on Alfworld \citep{shridhar2021alfworld}, 30\% on Textcraft \citep{prasad2024adaptasneededdecompositionplanning}, and 7\% on Webshop \citep{yao2023webshop}.  

Additionally, we validate that \textbf{StateAct} can serve as a drop-in replacement for existing extension methods. Using test-time computation \citep{prasad2024adaptasneededdecompositionplanning}, we achieve a further 12\% performance gain with StateAct on Textcraft compared to ReAct.  


==> sections/7_conclusion_previous.tex <==
% %%%%%%%%%%%%%%%
% Conclusion
\section{Conclusion and future work}
Our work is inspired by the challenge that LLMs and LLM agents struggle with long context and keeping on track with instructions. The current state-of-the-art to overcome such challenges propose extension on top of the base agent, ReAct. In contrast, we propose a new base agent StateAct, based on \textit{chain-of-states} and \textit{self-prompting}. Self-prompting is a novel contribution for LLM agents to prompt themselves with important cues such as the original instruction and goal. Chain-of-states is 

StateAct outperforms the previous best base agent, ReAct, between 9\%  and 20\% given different models and tasks. We validate that StateAct scales with extension methods, such as test-time compute. 

% In our analysis, we show that \textit{state-tracking} and \textit{self-prompting} can help the model solve long range reasoning tasks and interestingly also make the model more efficient.


 

% We found that `thoughts' or explicit reasoning do not always help performance. It would be very interesting to systematise `thought' and `states' and to understand what contributes positively and the reasons why. Also, inspired by the positive results of StateAct, it is interesting to see what other improvements can be made without resorting to training, larger models or external tools. Finally, problems related to \textit{domain-specific} syntax are also an interesting avenue for future work.


==> sections/abstract_previous.tex <==
\begin{abstract}
% Planning and acting to solve `real' tasks u
Using large language models (LLMs) in interactive environments has become a new frontier for AI research. Recent advances turn LLMs into LLM-agents that interact with websites, solve robotics tasks and play complex games.
% other tasks requiring strategic reasoning.
Existing LLM agent methods consist of a \textit{base agent} and optional extensions such as retrieval augmented generation (RAG), test time computation or additional training. In our work we propose StateAct,
% Existing methods to improve these AI Agents are often very resource-intensive and require additional data, additional computation, retrieval augmented generation (RAG) or human-crafted rules; instead, we propose StateAct, 
a new LLM base agent that is both efficient to run and outperforms the previous best-in-class. The main innovations are: 1. \textit{self-prompting} a method for the LLM to prompt itself with relevant cues and 2. enhancing \textit{chain-of-thought} with state-tracking.  
% StateAct is a base agent, similar to ReAct, and can be used with extensions such as RAG and test-time scaling. 
We outperform the current state-of-the-art base agent, ReAct, across a variety of tasks and 8 frontier models of different sizes. StateAct beats ReAct on average by over 10\% Alfworld, over 30\% on Textcraft and over 7\% on Webshop.
Additionally, we demonstrate that StateAct can be used as a drop-in replacement for ReAct and achieve a 12\% higher score using test time computation. \textbf{We release our code at URL}\footnote{URL is anonymised for submission.}.
% We also demonstrate that StateAct allows the agent to both solve longer horizon problems and to be more efficient in the number of steps required to solve a task. 
% Finally, 
% We open-source our code and annotations at \url{https://github.com/ai-nikolai/StateAct}.
\end{abstract}

==> sections/archive.tex <==


% Furthermore, StateAct even outperforms AdaPlanner by 2.48 points, an approach that uses regex for command-mapping (similar to our correction) along with using code-execution. 

% Perhaps the most surprising finding is that the simple correction described in Section \ref{sec:alfworld_correction} leads to a 16- and 23-point jump for ReAct and a 27-point jump for StateAct. This indicates that the model generally performs very well; however, it struggles with minute differences in \textit{domain-specific} syntax. 

% We also see that even without correction our method performs significantly better than strong baselines that are in context learning based, ReAct and AdaPlanner without code execution. We achieve 62.96, a 11 point jump to the closest system. In this case we find that StateAct without thoughts performs best. Since thoughts are verbose, this strengthens the hypothesis that more text based tokens harm \textit{domain specific} syntax.



% \begin{table}[t]
% \begin{tabular}{|l | c |} 
%  \hline
% \textbf{Method}&\textbf{SR \%}\\
% \hline
%  \hline
% \textit{Baselines}&\\
% \hline
% Act-only&41.48\\
% ReAct (Thought + Action) &63.70\\

% \hline 
% \textit{Our Methods}&\\
% \hline
% StateAct (State + Action) & 51.85 \\
% StateAct (Self-prompting + ReAct) & 64.44  \\
% StateAct (Self-prompting+State+Action) & 64.44  \\
% StateAct (Self-prompting+State+ReAct) &\textbf{77.04}\\
% \hline
% \end{tabular}
% \caption{Success Rate (SR) on the 134 test-set examples from Alfworld. The model was gpt-3.5-turbo-1106 with temperature 0.
% % *StateAct (complete) means self-prompting + state + thought + action. 
% All results are single run.}
% \label{tab:results_alfworld}
% \end{table}

% \begin{table}[t]
% \begin{tabular}{|l | c | c |} 
%  \hline
% \textbf{Method}&\textbf{GPT-3.5}&\textbf{SR \%}\\
% \hline
%  \hline
% \textit{Baselines}&&\\
% \hline
% Act-only&1106&41.48\\
% ReAct&1106&63.70\\
% % ReAct&0301*&\textbf{68.15}\\
% % AdaPlanner-base-agent** &0301*&46.66\\
% \hline 
% \textit{Our Methods}&&\\
% \hline
% State + Action & 1106&\textbf{64.44} \\
% Self-prompting + ReAct & 1106&\textbf{64.44} \\
% StateAct (ours) &1106&\textbf{77.04}\\
% -  w/o thought&1106&64.44 \\
% -  w/o goal&1106&74.04 \\
% -  w/o state&1106&64.44 \\
% \hline
% \end{tabular}
% \caption{Success Rate (SR) on the 134 test-set examples from Alfworld. *gpt-3.5-0301 was deprecated in June 2024. **AdaPlanner-base-agent means AdaPlanner without code execution (i.e. just the base agent). AdaPlanner results are from \citet{Sun2023AdaPlannerAP}. All other results are single run.}
% \label{tab:results_alfworld}
% \end{table}

% \begin{table}[t]
% \begin{tabular}{|l | c | c |} 
%  \hline
% \textbf{Method}&\textbf{GPT-3.5}&\textbf{SR}\\
% \hline 
% \textit{Baselines with Correction}&&\\
% \hline
% ReAct&0301*&68.15\\
% ReAct&1106&63.70\\
% AdaPlanner No-Exec** &0301&46.66\\
% AdaPlanner&0301*&75.56\\
% \hline 
% \textit{Results with Correction}&&\\
% \hline
% StateAct (ours) &1106&\textbf{77.04}\\
% -  w/o thought&1106&64.44 \\
% -  w/o goal&1106&74.04 \\
% -  w/o state&1106&64.44 \\
% \hline
% \end{tabular}
% \caption{Success Rate (SR) on the 134 test-set examples from Alfworld. *gpt-3.5-0301 is scheduled to be deprecated in June 2024. **No-Exec means AdaPlanner without code execution. ***joined ReAct means that \texttt{thought + action} are produced at every turn c.f. Figure
%  \ref{fig:method_prompt_comparison}.}
% \label{tab:results_alfworld_correction}
% \end{table}







% Interestingly, we see that removing thought produces the highest results and outperforms ReAct by 10 points. 
% Our hypothesis is that \textit{domain-specific} syntax, which is more prevalent in Webshop than Alfworld, conflicts with using verbose thoughts. 
% We therefore ran additional ablations where we only keep one of goal, state and thought. Table \ref{tab:results_webshop_ablation} demonstrates that thought seems to harm the performance the most while state seems to help the performance the most.

% \begin{table}[t]
% \begin{tabular}{|l | c |} 
%  \hline
% \textbf{Method}&\textbf{SR \%}\\
% \hline
%  \hline
% \textit{Baselines}&\\
% \hline
% Rule-based*&9.60\\
% RL* &17.60\\
% Act-only&39.00\\
% ReAct (Thought + Action) &36.00\\

% \hline 
% \textit{Our Methods}&\\
% \hline
% StateAct (State + Action) & 38.00 \\
% StateAct (Self-prompting + ReAct) & \textbf{40.00}  \\
% StateAct (Self-prompting+State+Action) & 38.00  \\
% StateAct (Self-prompting+State+ReAct) &37.00\\
% \hline
% \end{tabular}
% \caption{Success Rate (SR) on the 100 test-set examples from Webshop. *results taken from \cite{yao2023webshop}. The model was gpt-3.5-turbo-instruct with temperature 0. All results are single run. }
% \label{tab:results_webshop}
% \end{table}




% \begin{table}[t]
% \begin{tabular}{|l | c | c |} 
%  \hline
% \textbf{Method}&\textbf{GPT-3.5}&\textbf{Success Rate \%}\\
% \hline 
% \textit{Baselines}&&\\
% \hline
% Rule-based* &N/A&9.60\\
% RL* &N/A&17.60\\
% ReAct &1106&17.80\\
% % ReAct &0125&14.60\\
% % ReAct (joined) &1106&--\\
% \hline 
% \textit{Results}&&\\
% \hline
% StateAct (ours)&1106&17.00\\
% -  w/o thought&1106&\textbf{27.80}\\
% -  w/o goal&1106&20.40\\
% -  w/o state&1106&21.00\\
% \hline

% \hline 
% \textit{Ablations}&&\\
% \hline
% StateAct (State+Action)&1106&\textbf{28.40}\\
% \hline
% \end{tabular}
% \caption{Success Rate (SR) on the 500 test-set examples from Webshop. *results taken from \cite{yao2023webshop}. For StateAct without thought and ReAct Results are the average of two runs. Other Results are single run. }
% \label{tab:results_webshop}
% \end{table}



% \begin{table}[t]
% \begin{tabular}{|l | c |} 
%  \hline
% \textbf{Method}&\textbf{SR \%}\\
% \hline 
% % \textit{StateAct (ours)}&&\\
% % \hline
% React [joined] (Thought+Action)&18.00\\
% StateAct (ours) (Goal+Action)&26.60\\
% StateAct (ours) (State+Action)&\textbf{28.40}\\
% \hline
% \end{tabular}
% \caption{Success Rate (SR) on the 500 test-set examples from Webshop. Comparing each of goal, state and thought separately. All methods use gpt-3.5-1106.}
% \label{tab:results_webshop_ablation}
% \end{table}



% \begin{table}[h]
% \begin{tabular}{|l | c | c |} 
%  \hline
% \textbf{Method}&\textbf{Model}&\textbf{SR \%}\\
% \hline 
% \textit{Baselines}&&\\
% \hline
% ReAct &Gpt-3.5*&63.7\\
% ReAct &Gpt-4o-mini&68.15\\
% ReAct &Mixtral-8x22B**&72.59\\
% \hline 
% \textit{Results}&&\\
% \hline
% StateAct &Gpt-3.5*&77.04\\
% StateAct &Gpt-4o-mini&71.85\\
% StateAct &Mixtral-8x22B**&83.70\\
% \hline
% % \hline 
% % \textit{Ablations}&&\\
% % \hline
% % StateAct (State+Action)&1106&\textbf{28.40}\\
% % \hline
% \end{tabular}
% \caption{Success Rate (SR) on the 135 test-set examples from Alfworld. Results are `single run'. *=The concrete version of gpt-3.5 was gpt-3.5-1106.
% **=The concrete version of Mixtral is `mixtral-8x22b-instruct-v0.1'. 
% % StateAct** means (Self-prompt+State+Thought+Action).
% }
% \label{tab:results_additional}
% \end{table}

==> sections/archive/2_background.tex <==
% %%%%%%%%%%%%%%%
% Background
\section{Background}
While historically interactive tasks have  used reinforcement learning (RL) to solve tasks \cite{Sutton2018}, with the capabilities of LLMs improving, recent work has focused on using LLMs directly to solve these tasks \citep{yao2023react,li2022pretrained,Nottingham2023SelectivePO}.
% With the dawn of LLMs, works such as \citet{li2022pretrained,Nottingham2023SelectivePO} combines LLMs and RL and trained additional policies or value functions to make predictions. 

% It \citet{rana2023sayplan, Yao2023TreeOT,song2023llmplanner}

% \subsection{LLM based agents}
% Using the in-build world- and commonsense-knowledge of large language models \cite{lauscher-etal-2020-common} to perform interactive reasoning tasks (i.e. using LLMs as AI Agents) has become a frontier in AI research \cite{li2022pretrained, rana2023sayplan, singh2022progprompt, yao2023react}.

% Simulated environments, such as Alfworld \cite{shridhar2021alfworld} for house-hold robotics or Webshop \cite{yao2023webshop} for online shopping, are the testing bed of these capabilities.


% \cite{li2022pretrained} was among the first works to use LMs as environment encoders and trained an additional "task specific" policy to predict actual actions. 
% \citet{huang2022language} \cite{huang2022inner,yao2023react, Yao2023TreeOT,rana2023sayplan,song2023llmplanner, chen2024llmstate, Sun2023AdaPlannerAP, Nottingham2023SelectivePO, Tanaka2022DiffGRLLD, Wu2024StateFlowEL, Bhat2024GroundingLF, Fu2024AutoGuideAG, singh2022progprompt}.
\subsection{In-context learning approaches}
\citet{huang2022language, huang2022inner} and \citet{singh2022progprompt} were among the first to use LLMs directly to act in an interactive environment; their method produces agent actions as output after receiving environment observations as input.

ReAct \cite{yao2023react}  took this work further by combining `acting` \cite{huang2022language} and `chain-of-thought` \cite{wei2023chainofthought}. ReAct is among the best performing base agents and is the defacto base agent for most other methods until today.

ExpeL \cite{zhao2023expel} uses additional training data to generate `insights' and `success trajectories' during training. At inference time, they look up the closest `success trajectories' as few-shot examples to the agent (as opposed to the fixed few-shot examples that we use) and augment them with these `insights' to perform the final inference. They achieve 59\% on Alfworld using retrieved `success trajectories' (as few-shot examples) + `insights' and 50\% using the same few-shot examples as ReAct + `insights'.

\subsubsection{In-context learning and additional tools}
The current best approach for in-context learning-based approaches in combination with additional tools is ProgPrompt \citep{singh2022progprompt} and follow-on work AdaPlanner \cite{Sun2023AdaPlannerAP}. AdaPlanner introduces a code-based prompt \cite{li2023chainofcode}. They use code-execution as an additional tool, by executing LLM generated code and feeding the results into the next LLM generation. The shortcoming of AdaPlanner is that it requires very complex human-crafted prompts that are hard to scale to new environments and it requires the additional step of code-execution.

\subsection{State tracking in LLM-based agents}
% \subsubsection{Training data based methods} 
Concurrent work to ours, AutoGuide \cite{Fu2024AutoGuideAG}, uses ReAct as the base agent as well as additional training data to create `state-aware' text-based guidelines for the LLM-agent; they then use a type of retrieval augmented generation (RAG) process to guide the decision making process. They embed the current observation as a summary (which they call `state-aware') and use an LLM to `look up' the relevant `state-aware' guideline, which is then fed into a final LLM to generate an action. Using training data and LLM-based RAG, they achieve 79.1\% on top of a ReAct agent on Alfworld. Their training and RAG approach could be used complementary to our StateAct LLM-agent\footnote{However, the cost of using RAG at every generation step could be significantly higher than our method.}. 

\citet{chen2024llmstate} propose state-tracking as a way to help the agent solve the task without training data. Their method differs to ours two-fold. Firstly, they employ a complex sequence of components working together (an LLM-based attention over the observations, an LLM-based compilation of a complex state and, finally, a prediction of a program). Secondly, their system involves execution of actual programs. Our method, on the other hand, requires a straightforward extension of `chain-of-thought' and uses a single LLM call to produce the state, thought and action. Additionally, we do not require program execution. 



\subsubsection{Fine-tuning approaches}
Previous fine-tuning approaches did not significantly enhance performance \cite{zhou2024enhancing, yao2023react, shridhar2021alfworld}. A concurrent work, however, ActRe \cite{yang2024react} achieves 83\% by fine-tuning gpt-3.5-1106 on additional training data.

\subsection{``Multi-Agent Conversation'' approaches}
A new trend is to use multiple LLMs concurrently to `chat' to one another to produce a result. A recent work in this direction by \citet{wu2023autogen} achieves 67\% on Alfworld.

\subsection{Joined rule and LLM-based agents}
StateFlow \cite{Wu2024StateFlowEL} uses Finite State Machines (FSMs) combined with LLMs to solve Alfworld. These FSMs are human expert-crafted states, transitions and rule-based heuristics, where the LLM is asked to perform limited tasks in each of the given states. While their performance is 82\% on Alfworld, we believe this result is more comparable to a rule-based `expert' than an LLM-based agent (notably close to 100\% can be achieved on Alfworld using hand-crafted `experts' \cite{shridhar2021alfworld}).

% \citet{Nottingham2023SelectivePO} train an additional reinforcement learning based value-function to select a subset of the observation space for the LLM to make decisions on, they use different evaluation benchmarks in robotics the game NetHack.

% \citet{Tanaka2022DiffGRLLD} Use graph representation and a graph difference model to compare the "world state" embedded as a graph to an internal "commonsense graph" extracted from the LLM, the action selection, as well as graph embeddings happen via additional neural networks, word embeddings such as Glove \cite{pennington-etal-2014-glove} and graph embeddings.


% Furthermore, they evaluate on the program-execution based VirtualHome \cite{puig2018virtualhome}, while we follow the previous SOTA and evaluate on Alfworld.\\

\subsection{Test time computation}
ADaPT \citep{prasad2024adaptasneededdecompositionplanning} and THREAD \citep{schroeder2024threadthinkingdeeperrecursive} use test time computation to produce better results. This line of work is in line with works such a tree-of-thought \citep{Yao2023TreeOT}, where during test time inference the AI Agent proposes several thoughts or actions in one go and another model (often the same LLM) evaluates these, the top k promising thoughts or actions are expended upon further in a beam search manner. ADaPT enhances this by having another agent adaptively choosing to expand more steps at every turn given on the success or failure of a given action, while THREAD on a high-level combines ADaPT's methodology into one agent that itself knows when to expand the search. These methods while exhibiting very promising results (including reaching 100\% with a high-compute budget) require up to 100x compute budget compared to standard chain-of-thought (or ReAct in the agent case) \citep{Yao2023TreeOT}.

\subsection{Approaches with multiple trials and environment feedback}
Works such as Reflexion \cite{shinn2023reflexion} or work by \citet{Sun2023AdaPlannerAP, yang2024embodied} are methods that perform several evaluations on the same test environments and perform learning loops (during evaluation) on these test-set environments to improve the score. While the score necessarily goes up (as only the failed environments are re-run), we do not dive into this as it does not compare to the actual agent performance; additionally, `reflection` can be used on top of most LLM-based agents (e.g. Reflexion uses ReAct as the base agent).


% \subsection{Other approaches}
% While there are various approaches that have strong performance on standard benchmarks such as Alfworld. The methods that use actual LLM-based agents to perform the task (and achieve strong results) are limited to methods such as ReAct \cite{yao2023react} (51\% on Alfworld) in addition there are methods such AdaPlanner that use the LLM-only and use code-execution (of the code produced by the LLM) to perform the task \cite{Sun2023AdaPlannerAP} (75\% on Alfworld). While other works use additional input or human-experts to perform the task. They either use training data and bigger models during the training as in AutoGuide \cite{Fu2024AutoGuideAG} (79.1\% on Alfworld), expert-crafted rules to outperform in the task such as StateFlow \cite{Wu2024StateFlowEL} (83.3\% on Alfworld) or closed-loop learning on the actual test set to gain performance on the test set itself such as Reflexion \cite{shinn2023reflexion} (90+\% on Alfworld). Our work (77\% on Alfworld) on the other hand is purely few-shot in-context learning based and requires a single LLM call to produce both state and action, therefore our work is as simple as ReAct, however, produces results that are +9\% - +14\% better than ReAct and we even out-perform more complex state-of-the-art code-execution based approaches.

% \subsection{Interactive Environments}
% \note{REMOVE from this part and make it shorter, make less defensive and just mention in the alfworld section.}
% The common environment that was used is VirtualHome \cite{puig2018virtualhome} (also a Household robotics environment). ReAct first replaced VirtualHome, as it requires the execution of "programs", with alfworld \cite{shridhar2021alfworld}, a household robotics environment that is purely text based. This mainly overcame the previous challenge that the LLM agents had to both overcome the "executability" challenge as well as the "correctness" challenge. Where "executability" refers to the Agent producing valid commands, while "correctness" measures the actual success in the environment. In alfworld \cite{shridhar2021alfworld} this challenge is massively reduced and the agent is mainly left to solve "correctness". In our work we also focus on alfworld to focus on the actual "correctness" of the agent. In addition, similar to ReAct, we also use Webshop \cite{yao2023webshop}, which simulates the online shopping experience. 

% \subsection{List of papers to cover.}
%         \begin{itemize}
%             \item \cite{Bhat2024GroundingLF}
%             \item \cite{Wu2024StateFlowEL}
%             \item \cite{Tanaka2022DiffGRLLD}
%             \item \cite{Fu2024AutoGuideAG}
%             \item They are the only ones that have a state as well. They have zero citations and use quite a different environment (that's not so easy to get started). \cite{chen2024llmstate}
%             \item \cite{Nottingham2023SelectivePO}
%             \item \cite{Sun2023AdaPlannerAP}
%             \item \cite{li2022pretrained} One of the first
%             \item \cite{huang2022inner} React predecessor
%             \item \cite{huang2022language} one of the first agents
%             \item \cite{yao2023react} React itself obviously
%             \item \cite{rana2023sayplan} Say Plan
%             \item \cite{song2023llmplanner} LLM Planner
%             \item \cite{singh2022progprompt}
%             \item \cite{shinn2023reflexion}
             
%         \end{itemize}

==> sections/archive/2_background_alternative.tex <==
\section{Background}

Recent advances in large language models (LLMs) have enabled their use as autonomous agents in interactive environments, replacing traditional reinforcement learning (RL) approaches \cite{Sutton2018, yao2023react, li2022pretrained, Nottingham2023SelectivePO}. LLM-based agents now tackle tasks in simulated environments such as Alfworld \cite{shridhar2021alfworld}, Webshop \cite{yao2023webshop}, and TextCraft.

\subsection{LLM-Based Agents and In-Context Learning}
LLM agents typically follow an in-context learning paradigm, where the model generates actions based on environment observations without additional training. Early works such as \citet{huang2022language, singh2022progprompt} demonstrated this capability, with ReAct \cite{yao2023react} introducing reasoning via chain-of-thought (CoT), establishing itself as a standard baseline.



\subsection{Enhancing LLM Agents: RAG, Tools, State Tracking, and Fine-Tuning}
Extensions of ReAct include ExpeL \cite{zhao2023expel}, which retrieves successful trajectories for few-shot prompting, and AutoGuide \cite{Fu2024AutoGuideAG}, which integrates retrieval-augmented generation (RAG) to provide state-aware guidelines. While these improve performance, they introduce additional computation and complexity.

Some approaches enhance in-context learning with external tools. ProgPrompt \cite{singh2022progprompt} and AdaPlanner \cite{Sun2023AdaPlannerAP} employ code execution for structured reasoning but require complex handcrafted prompts. Other methods focus on state tracking: \citet{chen2024llmstate} propose a multi-component system for environment awareness, whereas StateFlow \cite{Wu2024StateFlowEL} combines finite state machines with LLMs for structured decision-making.

Fine-tuning efforts, while generally yielding limited improvements \cite{zhou2024enhancing, yao2023react}, have shown promise in ActRe \cite{yang2024react}, which fine-tunes GPT-3.5 to achieve state-of-the-art results.

\subsection{Test-Time Computation and Multi-Agent Collaboration}
Test-time computation methods such as ADaPT \citep{prasad2024adaptasneededdecompositionplanning} and THREAD \citep{schroeder2024threadthinkingdeeperrecursive} expand search steps adaptively, improving performance at the cost of significantly higher compute requirements. Multi-agent conversation approaches, where multiple LLMs collaborate (e.g., AutoGen \cite{wu2023autogen}), have also emerged as an alternative.

\subsection{Reflection-Based and Iterative Learning Approaches}
Some methods refine decisions by iterating within test environments. Reflexion \cite{shinn2023reflexion} and similar works \cite{Sun2023AdaPlannerAP, yang2024embodied} iteratively adjust actions based on previous failures, improving test-set performance but deviating from pure agent-based evaluations.

\subsection{Summary}
While various enhancements improve LLM-agent capabilities, many require additional computation, retrieval, fine-tuning, or handcrafted rules. Our work introduces \textbf{StateAct}, an efficient base agent that leverages self-prompting and state-tracking to outperform existing methods without additional overhead, achieving strong results across multiple tasks.

\begin{table}[h]
    \centering
    \begin{tabular}{|l|c|}
        \hline
        \textbf{Method} & \textbf{Score} \\
        \hline
        ReAct (few-shot only) & 63.7 \\
        AutoGuide (ReAct + RAG)* & 79.1 \\
        ActRe (ReAct + fine-tuning)** & 83.0 \\
        ADaPT (ReAct +Test time scaling)*** & 71.6 \\
        \hline
        % \textbf{StateAct (ours, few-shot only)} & \textbf{77.04} \\
        % \hline
    \end{tabular}
    \caption{Comparison of different methods using ReAct as base agent on Alfworld using gpt-3.5 level models. ReAct score is single run with greedy decoding using gpt-3.5-1106. *=\citep{Fu2024AutoGuideAG}, **=\citep{yang2024react}, ***=\citep{prasad2024adaptasneededdecompositionplanning}.}
    \label{tab:results_react}
\end{table}

